Label Shift Estimators for Non-Ignorable Missing Data

We consider the problem of estimating the mean of a random variable Y subject to non-ignorable missingness, i.e., where the missingness mechanism depends on Y . We connect the auxiliary proxy variable framework for non-ignorable missingness (West and Little, 2013) to the label shift setting (Saerens et al., 2002). Exploiting this connection, we construct an estimator for non-ignorable missing data that uses high-dimensional covariates (or proxies) without the need for a generative model. In synthetic and semi-synthetic experiments, we study the behavior of the proposed estimator, comparing it to commonly used ignorable estimators in both well-specified and misspecified settings. Additionally, we develop a score to assess how consistent the data are with the label shift assumption. We use our approach to estimate disease prevalence using a large health survey, comparing ignorable and non-ignorable approaches. We show that failing to account for non-ignorable missingness can have profound consequences on conclusions drawn from non-representative samples.

==> figures/case-study/error-table-clipped.tex <==
\begin{tabular}{llllll}
\toprule
   & method &                 cc &            cdirect &               cipw &             cproxy \\
{} & {} &                    &                    &                    &                    \\
\midrule
CO & bloodpressure &  0.223 [0.22-0.23] &  0.122 [0.12-0.13] &  0.114 [0.10-0.13] &  0.073 [0.06-0.08] \\
   & diabetes &  0.285 [0.28-0.29] &  0.213 [0.21-0.22] &  0.178 [0.16-0.20] &  0.234 [0.22-0.25] \\
   & cholesterol &  0.128 [0.12-0.13] &  0.106 [0.10-0.11] &  0.121 [0.11-0.13] &  0.114 [0.10-0.13] \\
   & depression &  0.182 [0.18-0.19] &  0.143 [0.13-0.15] &  0.184 [0.17-0.20] &  0.278 [0.26-0.29] \\
UT & bloodpressure &  0.210 [0.20-0.21] &  0.076 [0.07-0.08] &  0.128 [0.11-0.15] &  0.152 [0.14-0.16] \\
   & diabetes &  0.190 [0.18-0.20] &  0.071 [0.07-0.08] &  0.200 [0.17-0.23] &  0.364 [0.34-0.39] \\
   & cholesterol &  0.172 [0.17-0.18] &  0.095 [0.09-0.10] &  0.138 [0.12-0.16] &  0.159 [0.15-0.17] \\
   & depression &  0.285 [0.28-0.29] &  0.170 [0.16-0.18] &  0.298 [0.27-0.33] &  0.140 [0.12-0.16] \\
\bottomrule
\end{tabular}


==> sections/app-methods.tex <==
\subsection*{Missing Labels}
Define variables $(W, X, Y, M)$ from a source distribution $P(W, X, Y, M)$, where
\begin{itemize}
    \item $W \in \mathbb{R}^P$ --- subject level covariates
    \item $X \in \mathbb{R}^D$ --- waveform observation 
    \item $Y \in \{0, 1, \dots, K\}$ --- outcome 
    \item $M \in \{0, 1\}$ --- measurement indicator, $1$ when observed
    \item $S = m(X) \in \mathbb{R}^K$ ---
 scores for some deterministic predictive model $m: \mathbb{R}^D \mapsto \mathbb{R}^K$.
\end{itemize}
We only get to observe a samples $(W, X, Y) \sim P(W, X, Y \,|\, M = 1)$.  Further, we assume missing at random (i.e., ignorability), that is $X, Y \perp M \,|\, W$, that is, $W$ describes all the information needed to predict if the observation should be missing or not.  We also assume overlap, that is $P(M = 1 \,|\, W)$ is non-zero whenever $P(M=0 \,|\, W)$ is non-zero. 

One estimand of interest is simply the expectation of a loss function taken against the missing data distribution, e.g., 
\begin{align}
    \tau^{(mis)} &= \mathbb{E}_P\left[ f(X, Y) \,|\, M = 0 \right]
\end{align}
for some test function $f(X, Y)$ (e.g., mis-classification indicator or loss with respect to some prediction model $m(X)$).  

\paragraph{Estimating $\tau^{(mis)}$}
Intuitively, we can use the covariate vector $W$ to ``reconstruct'' the missingness indicator in expectation.  The goal is to derive an expression for this expectation that depends only on the observed data distribution --- that is when $M=1$. 

We can derive this expression (all expectations are with respect to $P$)
\begin{align}
    \tau^{(mis)} &= \mathbb{E}_{X,Y,W \sim P(X,Y,W | M=0)} \left[ f(X, Y) \,|\, M = 0 \right] \\
    &= \mathbb{E}_{W \sim P(W|M=0)}\left[\mathbb{E}_{X,Y \sim P(X,Y | M=0, W)} \left[ f(X, Y) \,|\, M=0, W \right] \right]\\
    &= \mathbb{E}_{W \sim P(W|M=0)}\left[\mathbb{E}_{X,Y \sim P(X,Y | W)}\left[ f(X, Y) \,|\, W \right]\right]  \text{\;\;\;\;\;\;\;\;\;\;(ignorability)} \\
    &= \frac{1}{P(M=0)} \int \mathbb{E}_{X, Y \sim P(X,Y |W)} \left[\frac{P(M=1|W)P(W)}{P(M=1|W)P(W)}f(X,Y) | W\right] P(W|M=0) P(M=0) dW \\
    &= \frac{1}{P(M=0)} \int \mathbb{E}_{X, Y \sim P(X,Y |W)} \left[\frac{P(W|M=0)P(M=0)}{P(M=1|W)P(W)}f(X,Y) | W\right] P(M=1|W) P(W) dW \\
    &= \frac{1}{P(M=0)} \mathbb{E}_{W \sim P(W|M=1)} \left[ \mathbb{E}_{X, Y \sim P(X,Y \,|\, W)} \left[ \frac{P(M=0|W)}{P(M=1|W)}f(X,Y) \,|\, W \right] P(M=1) \right] \\
    &= \mathbb{E}_{X, Y, W \sim P(X,Y,W | M=1)} \left[ \frac{P(M=0|W)}{P(M=1|W)}f(X,Y) \,|\, M=1 \right] \frac{P(M=1)}{P(M=0)} \label{eq:missing-tau}
    % P(X, Y, W) f(X, Y) dX dY dW  \\
    % &= \int \frac{P(M=1)}{P(M=1)}\frac{P(M=1 \,|\, W)}{P(M=1 \,|\, W)} P(X, Y, W) f(X, Y) dX dY dW  \\
    % &= \int \underbrace{\frac{P(X,Y, W, M=1)}{P(M=1)}}_{P(X,Y,W\,|\,M=1)} \frac{P(M=1)}{P(M=1 \,|\, Z)} f(X, Y) dX dY dW \\
    % &= \mathbb{E}\left[ \frac{P(M=1)}{P(M=1 \,|\, W)} f(X, Y) \,|\, M=1 \right] \\
    % &= \mathbb{E}\left[ \frac{1}{P(M=1 \,|\, W)} f(X, Y) \,|\, M=1 \right] \cdot P(M=1) \label{eq:missing-tau}
\end{align}
and we can derive an estimator for Eq.~\ref{eq:missing-tau} from our observed data
\begin{align}
    \hat{\tau}^{(mis)} &= \frac{\hat{p}_{m}}{1-\hat{p}_{m}} \frac{1}{N}\sum_{n=1}^N \frac{1-\hat{e}(w_n)}{\hat{e}(w_n)} f(x_n, y_n) \,\,, \quad x_n, y_n, w_n \sim P(X, Y, W \,|\, M=1) \label{eq:ipw-tau}
\end{align}
where $\hat{e}(w_n)$ is our propensity score estimate of $P(M=1 \,|\, W=w_n)$ and $\hat{p}_{m}$ is a plug in estimate of $P(M=1)$. 

\begin{aside}
Attempt at a more succinct derivation --- indicating conditional expectations as $\mathbb{E}_{X}[\cdot \,|\, W]$ against distribution $P(X \,|\, W)$
\begin{align*}
\tau^{(mis)} &= \mathbb{E}_{X,Y}\left[ f(X, Y) \,|\, M = 0 \right] \\
    &= \mathbb{E}_W\left[ \mathbb{E}_{X,Y}\left[ f(X, Y) \,|\, W, M=0 \right] \,|\, M = 0 \right] && \text{iterated expectations} \\
    &= \mathbb{E}_W\left[ \mathbb{E}_{X,Y}\left[ f(X, Y) \,|\, W \right] \,|\, M = 0 \right] && \text{ignorability} \\
    &= \mathbb{E}_W\left[ \tfrac{P(W \,|\, M=0)}{P(W \,|\, M=1)}\mathbb{E}_{X,Y}\left[ f(X, Y) \,|\, W \right] \,|\, M = 1 \right] && \text{importance re-weighting}\\
    &= \mathbb{E}_W\left[ \tfrac{P(M=0 \,|\, W)}{P(M=1 \,|\, W)} \tfrac{P(M=1)}{P(M=0)} \mathbb{E}_{X,Y}\left[ f(X, Y) \,|\, W \right] \,|\, M = 1 \right] && \text{mult.~$\tfrac{P(M=0)}{P(M=0)}\tfrac{P(M=1)}{P(M=1)}$}\\ 
    &=\tfrac{P(M=1)}{P(M=0)} \mathbb{E}_{W,X,Y}\left[ \tfrac{P(M=0 \,|\, W)}{P(M=1 \,|\, W)} f(X, Y) \,|\, M = 1 \right] && \text{rearrange,}
\end{align*}
motivating the estimator 
\begin{align}
    \hat{\tau}^{(mis)} &= \frac{\hat{p}_{m}}{1-\hat{p}_{m}} \frac{1}{N}\sum_{n=1}^N \frac{1-\hat{e}(w_n)}{\hat{e}(w_n)} f(x_n, y_n) \,\,, \quad x_n, y_n, w_n \sim P(X, Y, W \,|\, M=1) \label{eq:ipw-tau}
\end{align}
\end{aside}

\begin{aside}
Note: There probably exists a simple doubly robust extension to this estimator that uses a model prediction $\mathbb{E}\left[Y \,|\, X, M=1 \right]$, i.e., the prediction model.  Not sure how to extend this to the generic test function $f(X, Y)$, but maybe it's a two step plugin. 
\end{aside}

\begin{aside}
Ignorability implies ignorability of the propensity score --- it suffices to show that $\mathbb{E}[M \,|\, W, e(W)] = \mathbb{E}[M \,|\, e(W)]$.  The left side reduces to
\begin{align}
    \mathbb{E}[M \,|\, W, e(W)] = \mathbb{E}[M \,|\, W] \triangleq e(W) \,
\end{align}
because $e(W)$ is a determinstic random variable. 
The right side reduces to 
\begin{align}
    \mathbb{E}[M \,|\, e(W)] &= P(M=1 \,|\, e(W)) \cdot 1 + P(M=0 \,|\, e(W)) \cdot 0 \\
    &= P(M=1 \,|\, e(W)) \\
    &= e(W) \,
\end{align}
so $e(W)$ contains all the information in $W$ about $M$.

\end{aside}



So this suggests a concrete approach for estimating $\tau^{(mis)}$: 
\begin{itemize}
    \item Fit a well-calibrated propensity score model $\hat{e}(w) = Pr(M = 1 \,|\, W=w)$.  This can be done with whatever classifier, and probably some sort of post-hoc calibration procedure (like Platt Scaling). 
    \item Compute the empirical missing probability $\hat{p}_m$, i.e., the fraction of missing targets from the source distribution.  This, of course, assumes you have (or know the size of) unlabeled data.
    \item Compute the re-weighted average in Eq.~\ref{eq:ipw-tau}.
\end{itemize}
One can repeat this procedure for multiple bootstrap replicates of the test data (which includes re-training and calibrating a propensity score model) to get confidence intervals.


\subsection*{Distribution Shift}
As alluded to, our real goal is to estimate a quantity with respect to a target distribution $Q$ --- e.g., the entire US population.  So we may have to cope with both the missing label issue \emph{and} an additional distribution shift. 

Our goal is to compute an expectation 
\begin{align}
    \tau_Q^{(mis)} = \mathbb{E}_{Q} \left[ f(X, Y) \,|\, M = 0 \right]. 
\end{align}
In words, this is the performance of a model on the target distribution $Q$ for unmeasured individuals. 
Given a sample from $P$, the typical strategy to estimate this quantity using a re-weighted average
\begin{align}
    \tau_Q^{(mis)} &= \mathbb{E}_{Q} \left[ f(X, Y) \,|\, M = 0 \right] \\ 
    &= \mathbb{E}_{P} \left[ \frac{Q(X, Y \,|\, M=0)}{P(X, Y \,|\, M=0)} f(X, Y) \,|\, M = 0 \right]
\end{align}

To gain traction on this problem, we need to observe some data from the distribution $Q$ and/or make assumptions about how they relate to each other. 

In our setting, we will make additional assumptions
\begin{itemize}
\item \textbf{Covariate and label stability} --- this assumes that $P(X \,|\, Y, W) = Q(X \,|\, Y, W)$ --- that is our physiological measurement is the same in source and target, given enough information about the subject. 
\item \textbf{Missingness stability} --- this assumes that $P(M=1 \,|\, W) = Q(M=1 \,|\, W)$ --- that is, the mechanism that induces missing labels in our source sample is the same in our target sample given subject covariate  information. 
\item \textbf{Target ignorability} --- we extend ignorability to the target distribution as well, $(X,Y) \perp M \,|\, W$ under $Q$. 
\end{itemize}

These assumption implies that our source and target distributions share some structure:
\begin{align}
  P(X, Y, W) = P(X \,|\, Y, W) P(Y, W) \\
  Q(X, Y, W) = P(X \,|\, Y, W) Q(Y, W)
\end{align}
i.e., the signal $X$ is generated the same way in both populations, given the covariate information. 

Now we can write an estimate of $\tau_Q^{(mis)}$ in terms of the observed source distribution
\begin{align}
    \tau_Q^{(mis)} &= \mathbb{E}_{Q} \left[ f(X, Y) \,|\, M = 0 \right] \\ 
    &= \mathbb{E}_{Q}\left[ \mathbb{E}_{Q} \left[ f(X, Y) \,|\, M = 0 \right] | W \right] \\
    &= \mathbb{E}_{P} \left[ \frac{Q(X, Y, W \,|\, M=0)}{P(X, Y, W\,|\, M=0)} f(X, Y) \,|\, M = 0 \right] \\
    &= \mathbb{E}_{P} \left[ \frac{P(X \,|\, Y, W, M=0) Q(Y\,|\, W, M=0)}{P(X, Y, W\,|\, M=0)} f(X, Y) \,|\, M = 0 \right]
\end{align}

\begin{aside}
Note that the Covariate and label stability assumption is weaker than the often-used label-shift assumption, which assumes $P(X \,|\, Y) = Q(X \,|\, Y)$.  Here we allow for additional demographic factors to influence both the signal $X$ and the outcome $Y$. 
\end{aside}



\section*{Doubly Robust Estimators for Missing Data}
Doubly robust estimators are most typically presented for estimating the population mean or the average treatment effect (ATE) for problems where data are missing.  These estimators typically combine estimates of $E[Y \,|\, W, M=1]$ and the IPW expectation $E[ \frac{1}{e(W)} Y \,|\, M = 1]$ to construct a doubly robust estimate of $E[Y]$ in the complete data setting.  

Our situation is a bit more complicated, as we want to estimate $E[f(X, Y)]$ or $E[f(X, Y) \,|\, M=0]$ for some test function $f$.  The question is, do these methods easily/directly translate to our situation? 

The trick might be to simply unpack $f(X, Y)$ into particular targets of interest.  
For example, say we care about the true positive rate
\begin{align}
    f(X, Y) &= \mathbbm{1}(m(X) > t_0) \mathbbm{1}(Y = 1)\\
    \mathbb{E}(f(X, Y)) &= Pr(m(X) > t_0, Y=1)
\end{align}






\section*{Binary Method of Moments Derivation}

Given this assumption, we see that $\beta_0$ and $\beta_1$ are shared across levels of $M$, leaving only $\mu_Y^{(1)} = \mathbb{E}[Y \,|\, M=1]$ to be identified.

We can derive an estimator by matching two ways to compute the expectation of $X$ when $M=1$.  The first is straightforward --- we observe $X$ when $M=1$ so we can just compute the sample mean
\begin{align}
    \mathbb{E}[X \,|\, M=1] = \mu_X^{(1)} 
    \approx \hat{\mu}_{X}^{(1)} \,,
\end{align}
and we can apply the tower law to relate the estimator to $Y$
\begin{align}
    \mathbb{E}[X \,|\, M=1] 
    &= \mathbb{E}[ \mathbb{E}[ X \,|\, Y] \,|\, M=1] \\
    &= \mathbb{E}[ \beta_0 \cdot (1 - Y) + \beta_1 \cdot Y \,|\, M=1] \\
    &= \beta_0 \cdot (1 - \mathbb{E}[Y \,|\, M=1]) + \beta_1 \cdot \mathbb{E}[Y \,|\, M=1] \\
    &= \beta_0 \cdot (1 - \mu_Y^{(1)}) + \beta_1 \cdot \mu_Y^{(1)} \\
    &= \beta_0 + (\beta_1 - \beta_0) \cdot \mu_Y^{(1)}
\end{align}
This implies 
\begin{align}
    \mu_X^{(1)} &= \beta_0 + (\beta_1 - \beta_0) \cdot \mu_Y^{(1)} \\
    \implies 
    \mu_Y^{(1)} &= \frac{\mu_X^{(1)} - \beta_0}{\beta_1 - \beta_0} \,,
\end{align}
where all of the quantities on the right side can be estimated from data --- we can plug the maximum likelihood estimator in for each quantity. 
Further, we can algebraically manipulate the right hand side to relate the estimator to the observed mean $\mu_Y^{(0)}$.  By symmetry, for the case $m=0$ we have 
\begin{align}
    \mu_Y^{(0)} = \frac{\mu_X^{(0)} - \beta_0}{\beta_1 - \beta_0} \implies 
    \beta_1 - \beta_0 = \frac{\mu_X^{(0)} - \beta_0}{\mu_Y^{(0)}} 
\end{align}
and plugging this into the above yields
\begin{align}
    \mu_Y^{(1)} &= \frac{\mu_X^{(1)} - \beta_0}{\mu_X^{(0)} - \beta_0} \cdot \mu_Y^{(0)} \,.
\end{align}
This formula directly shows the adjustment made to the observable mean value $\mu_Y{(0)}$ based on an adjusted ratio of the missing population $\mu_X^{(1)}$ and the complete cases $\mu_X^{(0)}$, and how it relates to $\beta_0 = P(X=1 \,|\, Y=0)$.
Plugging the MLE estimates for each quantity on the right hand side gives us our first estimator, which we refer to as the method of moments estimator.


\subsection{Maximum likelihood estimator}
% The pattern mixture factorization describes the conditional distribution of variables $X, Y$ given response, e.g., 
% \begin{align}
%     X, Y \,|\, \{M=m\} \sim p(X, Y ; \theta^{(m)})
% \end{align}
% where $\theta^{(m)}$ describes the joint distribution over two binary variables, i.e., with three degrees of freedom. 
% We can describe this joint as a marginal of $Y$ and conditional $X \,|\, Y$
% \begin{align}
%     Y &\sim \texttt{Bern}(\mu_Y) \\
%     X \,|\, Y &\sim \texttt{Bern}(\beta_0 \cdot (1 - Y) + \beta_1 \cdot Y) 
% \end{align}
% with $\beta_0, \beta_1, \mu_Y \in [0, 1]$, and we denote $\theta = (\mu_Y, \beta_0, \beta_1)$.
% For two levels of missingness we have $\theta^{(0)}$ and $\theta^{(1)}$, as well as the marginal missingness probability $P(M=1) = \pi$, yielding seven unknown parameters.
% It is clear that $\theta^{(0)}$ and $\pi$ are identifiable from the sample data alone, and parameters $\theta^{(1)}$ are not identified from observations alone.

We noted previously that this non-ignorable missing data estimator is similar to the label shift problem. 
We can also derive a ma
The log likelihood can be written
\begin{align}
    \ln \ell(\theta) 
    &= \ln \left(
        \prod_n P(m_n \,|\, \pi) 
        \prod_{n \in \mathcal{I}_{obs}} P(y_n \,|\, \mu_Y^{(0)}) P(x_n \,|\, y_n, \beta) 
        \prod_{n \in \mathcal{I}_{mis}} P(x_n \,|\, \beta)
    \right) \\
    &= \sum_{n} \ln P(m_n \,|\, \pi) + 
       \sum_{n \in \mathcal{I}_{obs}} \ln P(y_n \,|\, \mu_Y^{(0)}) + \ln P(x_n \,|\, y_n, \beta) + 
       \sum_{n \in \mathcal{I}_{mis}} \ln P(x_n \,|\, \theta)
\end{align}
where the last term is the $x_n$ values 


==> sections/lit-review.tex <==


